AutoCheck: Automatically Identifying Variables for Checkpointing by Data Dependency Analysis

Checkpoint/Restart (C/R) has been widely deployed in numerous HPC systems, Clouds, and industrial data centers, which are typically operated by system engineers. Nevertheless, there is no existing approach that helps system engineers without domain expertise, and domain scientists without system fault tolerance knowledge identify those critical variables accounted for correct application execution restoration in a failure for C/R. To address this problem, we propose an analytical model and a tool (AutoCheck) that can automatically identify critical variables to checkpoint for C/R. AutoCheck relies on first, analytically tracking and optimizing data dependency between variables and other application execution state, and second, a set of heuristics that identify critical variables for checkpointing from the refined data dependency graph (DDG). AutoCheck allows programmers to pinpoint critical variables to checkpoint quickly within a few minutes. We evaluate AutoCheck on 14 representative HPC benchmarks, demonstrating that AutoCheck can efficiently identify correct critical variables to checkpoint.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> case_study.tex <==
\section{Case studies} 
\label{sec:case}
% \subsection{Use of AutoCheck in Different Inputs}
% Figure~\ref{fig:user_manual} shows how to use AutoCheck.
% % When using AutoCheck, users need to provide three things.
% Using AutoCheck requires as following.

% \begin{enumerate}
% \item
% Using LLVM-Tracer to generate dynamic instruction traces for source code that needs to identify critical variables.
% % \item
% main computation loop's beginning and end line numbers. 
% % \item
% What form does the main computation loop take in the main function? 
% If the loop appears in the main computation loop directly, you need to enter 0 to tell AutoCheck that the main computation loop is in the main function. 
% If the main computation loop is in another function, you need to enter the line number where this function is called in the main function.
% \end{enumerate}
% \begin{figure}
%   \begin{center}
%   \includegraphics[width=3.6in]{figure/use_of_autocheck.pdf}
%   %\vspace{-5pt}
%   \caption{User manual for AutoCheck}
%   \label{fig:user_manual}
%   \end{center}
%   \vspace{-20pt}
% \end{figure}
% }



We further evaluate \texttt{AutoCheck} on two large HPC proxy (MPI) applications, CoMD (5637 LOCs) and miniAMR (11531 LOCs), from the Exascale Computing Project (ECP) proxy application suite~\cite{sultana2021understanding}.
We describe the two applications in Table~\ref{tab:epc_benchmark_description}, including the application description, LOC, the input size used for LLVM trace generation, the generated trace size, and the cost of trace generation. 
We use the same experimental setup as used for the 10 benchmarks.
% \texttt{CoMD}: 
% A proxy application in molecular dynamics (MD), typically used as a research platform for particle motion simulations. Unlike previous MD proxy applications (e.g. MiniMD), CoMD is designed to be significantly modular, allowing for individual module analysis.
% \texttt{miniAMR}: 
% A software for octree-based adaptive mesh refinement (AMR) that can be used to study the communication costs in a typical AMR simulation.



\textbf{Validating detected variables to checkpoint. }
We report the \texttt{AutoCheck}-detected variables for checkpointing in Table~\ref{tab:epc_benchmark_cpk}. 
We use the same approach used before in Section~\ref{sec:validation} to validate the effectiveness of the detected variables for checkpointing. 
With the detected variables checkpointed, both CoMD and miniAMR restart successfully in a simulated fail-stop failure.
We also test the detected variables with different inputs, and find out that the execution restarts successfully in all cases.
In particular, for CoMD, we tried{} $20 \times 20 \times 20$ and $25 \times 25 \times 25$, for miniAMR, we tried $8 \times 8 \times 8 \times 4000$ and $8 \times 8 \times 8 \times 9000$.
This demonstrates the sufficiency (or completeness) of the detected variables for checkpointing and the capability of our analytic model to handle different inputs. 
To check the necessity (or exclusivity) of the detected variables, we turn off C/R to one of those variables at a time and see if the execution still restarts successfully and outputs correct results. 
To the end, we didn't find unnecessary (false-positive) variables in the detected variables.
% In consequence, we justified the effectiveness of \texttt{AutoCheck}-detected variables for CoMD and miniAMR. }




% We also observe that there are only two data dependency types found from the detected variables: Write-After-Read (WAR) and Index. 
% We hope that this can give some insights to future C/R studies on common dependency types for checkpointing. 

% shows the details of the variables that need to checkpoint for CoMD and miniAMR as well as the information about their corresponding dynamic instruction execution trace.
% Also, to verify the validity of the identified variables by \texttt{AutoCheck}, we have tried different large input sizes.
% we manually add C/R codes to application and simulate application running failure and restart the application.
% For CoMD, we tried{} $20 \times 20 \times 20$ and $25 \times 25 \times 25$, for miniAMR, we tried $8 \times 8 \times 8 \times 4000$ and $8 \times 8 \times 8 \times 9000$.
% All of our tests are restart successfully, and the results show that \texttt{AutoCheck} can effectively deal with large scale applications.



\textbf{Discussion.} There are in total 52 variables detected to checkpoint, where 49 are Write-After-Read, and 2 are Index.
Moreover, we found in miniAMR that many WAR variables that need to checkpoint take themselves from previous iterations as input, such as timers and counters.
We hope that those findings can give some insights to future C/R studies on common dependency types for checkpointing.
% themselves (i.e. they need to update their values in each iteration based on the value obtained in the previous iteration). 
% For example, timers and counters, which are updated based on themselves.
% In CoMD, there are three variables to checkpoint, 2 are  and one is index.
% In miniAMR, there are in total 49 variables to checkpoint. 47 are Write-After-Read, 2 are index. 




\textbf{Efficiency study.}
We report the analysis cost in Table~\ref{tab:ecp_time}.
% shows the analysis overhead of \texttt{AutoCheck} works with large-scale MPI applications.
\textcolor{orange}{Each measurement is averaged over five runs.
The total analysis time for CoMD is 2.1 minutes (3.7 seconds with optimization), while for miniAMR is 4.1 minutes (1.8 minutes with optimization). 
We look into the source code of CoMD and find out that there are more than 95\% instructions for initialization and logging and only less than 5\% instructions for the main computation loop.
That's why CoMD has a larger trace, but the analysis cost is much lower.}

% In particular, miniAMR has 11531 lines of code, and the dynamic instruction execution trace we generated using LLVM-Tracer is only 2.3G.
% Compared to manually identifying variables for checkpointing for  complex code, \texttt{AutoCheck}'s performance has amply demonstrated that it is very efficient.

\begin{comment}


\begin{table}[h!]
\begin{center}
\caption {HPC proxy applications for case studies.}
%\vspace{-5pt}
\label{tab:epc_benchmark_description}
%\tiny
\scriptsize
\begin{tabular}{|p{0.9cm}|p{2.65cm}|p{0.4cm}|p{0.5cm}|p{1.25cm}|}
\hline
\textbf{Name} 	& \textbf{Application description} 	& \textbf{LOC}  & \textbf{Trace size} & \textbf{Trace generation time (s)}             \\ \hline \hline
CoMD (ECP)             & A proxy application in molecular dynamics (MD) often used for particle motion simulations (input size $4 \times 4 \times 4$)     &5637  &3.4G    &59.37	  \\ \hline
miniAMR (ECP)            & A large-scale 3D stencil calculation by Adaptive Mesh Refinement (input size --$nx$ 2 --$ny$ 2 --$nz$ 2 --$max\_blocks$ 2)        &11531  &2.3G   &39   \\ \hline
\end{tabular}
\end{center}
% \vspace{-15pt}
\end{table}


\begin{table}[]
\begin{center}
\caption {Detected checkpointing variables for HPC proxy applications. WAR means ``\underline{W}rite-\underline{A}fter-\underline{R}ead''.}
%\vspace{-5pt}
\label{tab:epc_benchmark_cpk}
%\tiny
\scriptsize
\begin{tabular}{|p{0.9cm}|p{4.5cm}|p{0.9cm}|}
\hline
\textbf{Name} 	& \textbf{Variables to checkpoint (Dependency type)}  	& \textbf{Validation}             \\ \hline \hline
CoMD             &$sim$ (WAR), $perfTimer$ (WAR), $iStep$ (Index)	&\emph{successful}  \\ \hline
miniAMR   &29 $timers$ (WAR), $counter\_bc$ (WAR), $total\_fp\_adds$ (WAR),  $total\_blocks$ (WAR), $total\_fp\_divs$ (WAR), $total\_red$ (WAR),  $nrs$ (WAR), $nrrs$ (WAR),$num\_moved\_coarsen$ (WAR),  $num\_moved\_rs$ (WAR), $num\_comm\_uniq$ (WAR),  $num\_comm\_tot$ (WAR), $num\_comm\_z$ (WAR),  $num\_comm\_y$ (WAR), $tmax$ (WAR),$tmin$ (WAR),$global\_active$ (WAR),  $num\_comm\_x$ (WAR), $blocks$ (WAR), $done$ (Index),  $ts$ (Index)	&\emph{successful} \\ \hline
\end{tabular}
\end{center}
% \vspace{-10pt}
\end{table}

\begin{table}[]
%\vspace{-5pt}
%\tiny
\centering
\scriptsize
\caption{Efficiency study for HPC proxy applications. Optimization means parallel execution with 48 threads.}
\begin{tabular}{|p{0.85cm}|p{1.55cm}|p{1.07cm}|p{0.98cm}|p{1.3cm}|}
\hline
\textbf{Name}  	 & \textbf{Pre-processing (With optimization) (s)}	& \textbf{Dependency Analysis (s)} 	& \textbf{Identify Variables (s)}	 & \textbf{Total Time (With optimization) (s)}   \\ \hline \hline
CoMD     & 129.47  (3.71)   &2e-3      &5e-4     & 129.47 (3.71) \\\hline 
miniAMR      & 142.97  (4.21)   &105.23      &0.12      &248.32 (109.56) \\\hline 
%$hierarchy.levels[0].R.V$ \\ \hline
\end{tabular}
\label{tab:ecp_time}
% \vspace{-18pt}
\end{table}

\end{comment}



% \begin{table*}[h!]
% \begin{center}
% \caption {Benchmarks and applications for the study. LOC means ``\underline{L}ines \underline{O}f \underline{C}ode''; WAR means ``\underline{W}rite-\underline{A}fter-\underline{R}ead''; PO means ``\underline{P}artially-\underline{O}verwritten''.}
% %\vspace{-5pt}
% \label{tab:epc_benchmark}
% %\tiny
% \scriptsize
% \begin{tabular}{|p{1.1cm}|p{5.2cm}|p{0.4cm}|p{1cm}|p{1.4cm}|p{5.2cm}|p{0.9cm}|}
% \hline
% \textbf{Name} 	& \textbf{Application description} 	& \textbf{LOC}  & \textbf{Trace size} & \textbf{Trace generation time (s)}	& \textbf{Variables to checkpoint (Dependency type)}  	& \textbf{Validation}             \\ \hline \hline
% CoMD (ECP)             & A proxy application in molecular dynamics (MD) often used for particle motion simulations (input size $4 \times 4 \times 4$)     &5637  &3.4G    &59.37		&$sim$ (WAR), $perfTimer$ (WAR), $iStep$ (Index)	&\emph{successful}  \\ \hline
% miniAMR (ECP)            & A large-scale 3D stencil calculation by Adaptive Mesh Refinement (input size --$nx$ 2 --$ny$ 2 --$nz$ 2 --$max\_blocks$ 2)        &11531  &2.3G   &39 	&$29\ timers$ (WAR), $counter\_bc$ (WAR),  $total\_fp\_adds$ (WAR),  $total\_blocks$ (WAR),  $total\_fp\_divs$ (WAR),  $total\_red$ (WAR),  $num\_moved\_coarsen$ (WAR),  $num\_moved\_rs$ (WAR), $num\_comm\_uniq$ (WAR),  $num\_comm\_tot$ (WAR),  $tmin$ (WAR),  $num\_comm\_z$ (WAR),  $num\_comm\_y$ (WAR),  $blocks$ (WAR),  $global\_active$ (WAR),  $num\_comm\_x$ (WAR), $nrs$ (WAR),  $tmax$ (WAR),  $nrrs$ (WAR),$done$ (Index),  $ts$ (Index)	&\emph{successful} \\ \hline

% \end{tabular}
% \end{center}
% \vspace{-20pt}
% \end{table*}









% \textbf{MPI programs.}
% Different from serial cases,  we use \emph{mpicc} and \emph{mpirun} to compile and run LLVM-Tracer for MPI programs. 
% % and use  to execute this binary executable with only one MPI process.
% % We provide a table in the artifact description that details the difference between compilation commands used for serial and MPI programs.
% Table~\ref{tab:setup_for_mpi} compares the difference between compilation commands used for serial and MPI programs for trace generation, taking miniAMR as an example.
% The generated LLVM traces in both cases follow the same trace format as described in Section~\ref{sec:llvm-trace}.




% We have showcased that \texttt{AutoCheck} works for MPI programs with one rank. 

==> overview.tex <==
\section{Overview}

\begin{figure*}[ht]
  \begin{center}
  \includegraphics[width=0.85\textwidth,keepaspectratio]{figure/autocheck_workflow.pdf}
  %\vspace{-5pt}
%   \caption{AutoCheck workflow diagram. \az{remove "2) saved instructions"; change "1) matched variables" to "main-loop’s inputs variables"; change "Dependency between variables" to "DDG"}}
% \kt{It might be good to differentiate between "task (pre-processing)" and "data (e.g., main-loop inputs)" with different shape of boxes}
  \caption{\texttt{AutoCheck} workflow diagram. }
  \label{fig:tool_workflow}
  \end{center}
  \vspace{-1em}
%   \vspace{-20pt}
\end{figure*}


This section overviews the \texttt{AutoCheck} analytical model.
\texttt{AutoCheck} takes a dynamic instruction execution trace as input. 
\texttt{AutoCheck}'s workflow (as shown in Figure~\ref{fig:tool_workflow}) has three modules: pre-processing, 
data dependency analysis, and identification of variables to checkpoint.
% We describe the AutoCheck workflow in Figure~\ref{fig:tool_workflow}. 

% We introduce an analytical model to identify critical variables for checkpointing using dynamic trace analysis. 


% By studying the regularity of variables in dynamic instruction trace, we design and develop a tool for data dependency analysis. 
% The input of this tool is the dynamic instruction trace generated using LLVM-Tracer and the information of main computation loop. 
% Our tool reads the dynamic instructions trace twice, the first time is pre-processing, and the second time is preforming data dependency analysis. As described in the workflow diagram in Figure~\ref{fig:tool_workflow}, our analytical model includes the following steps. 

\subsection{Identifying MLI variables}
% Before any analytics, we first generate dynamic instruction execution trace using a trace generation tool, 
% LLVM-Tracer~\cite{shao2013isa}, which is an LLVM instrumentation pass that prints out a dynamic LLVM IR trace. 

We attempt to identify the main computation loop's input variables. Those variables are candidates for variables to be checkpointed. 
An input variable must be defined before but used in the main computation loop.
% We first read the input trace and store the dynamic instruction execution information into memory, and collect and output these variables defined before and used in the main computation loop. 
%we divide the trace into three parts based on the user input for the main loop: before the main loop, inside the main loop, and after the main loop. Next, we extract the variables that are defined before the main loop and used in the main loop. These variables are the output of the preprocessing.}
% \az{Summrize the preprocessing.}
% \az{main loop -> main computation loop.}
However, if the variable is defined before the main computation loop, but within a function call, we exclude it from our consideration.
% In particular, we exclude those variables defined locally in a function call, whose invocation appears before and within the main computation loop. 
Because those variables are local variables which cannot affect the global execution state. 
% With this way, we can identify the potential input variables to be checkpointed in the main computation loop.

% There are several challenges during this process. 
% First, if a local variable defined in function which called both the before and inside of the main loop, then this variable will also be extracted as part of the output during preprocessing. 
% But this variable is not necessary for data dependency analysis, it is only a local variable and does not affect the correct execution of the main loop. 
% So, we need to avoid obtaining the local variables that defined in the function called at the main loop.
\subsection{Data dependency analysis}
The data dependency analysis interface takes 
the MLI variables as input, and tracks the data dependency \emph{only} between those variables by \emph{selectively} passing the dynamic instruction execution information, meaning that we focus on arithmetic instructions (such as `\texttt{Fadd}') and complement instructions (such as `\texttt{Load}' and `\texttt{Store}') and transition instructions (such as `\texttt{Call}') for arithmetic instructions.
All data dependencies are refined and stored into a graph finally.

%, and finally saves the extracted data dependency into an ordered map
% \lhm{In the trace, we can only identify variable by register name, so we update the relationship between variables and their corresponding registers in real time during the process of dependency analysis, which is the core of data dependency analysis. Then we handle the instructions in the trace according to the opcodes of each one.}
There are several design and implementation difficulties to enable \emph{effective} analysis to the numerous dynamic instructions. 
Many of those difficulties result from the Static Single Assignment form (SSA), for which arithmetic variables participate in computations through temporary registers.
% , because of  (or SSA), and local variables, a complement to the main-loop's input variables. 
% The \emph{primary} difficulty to performing a \emph{complete} data dependency analysis, meaning that all arithmetic instructions and its complements and  along the execution flow are constructed into a \emph{complete DDG}, is that we must address data dependency propagation and transition between different entities, such as from arithmetic variables to temporary registers, from `Load' and `Store' instructions to arithmetic instructions, and from `Load' and `Store' instructions to function calls.
To address the difficulties because of SSA, we first identify the correlations between arithmetic variables and temporary registers from `\texttt{Load}' and `\texttt{Store}' instructions. 
Those correlations allow us to track the data dependency between arithmetic variables by temporary registers from arithmetic instructions, as 
arithmetic variables participate in computations (such as arithmetic operations and function calls) through temporary registers (because of SSA).
Likewise, the correlations between arithmetic variables and temporary registers allow us to track the data dependency propagation while entering and exiting a function call through the transition between function arguments and parameters. 
We construct \emph{a complete DDG that includes all those data dependencies, describing correlations between the main computation loop's input variables and other application state, including local variables and temporary registers.}

Finally, we propose a DDG contraction algorithm to \emph{contract} the \emph{complete DDG} until it contains the main computation loop's input variables \emph{only}, as those variables are candidates for checkpointing. 

\begin{comment}
involve these intermediate state, such as temporary registers, into data dependency analysis for a \emph{complete} data dependency analysis.
% \az{TODO: for which we construct a separate DDG to dynamically track and update the dependency between intermediate state (including temporary registers and local variables) and the main-loop’s inputs variables on the fly.
% % \kt{What is implication of using "integral" data dependency analysis ?}
% This separate DDG aids the construction of the primary DDG for the main-loop’s inputs variables. }
\lhm{Therefore, we extract the correlation between single variables and temporary registers by 'Load' and 'Store' instructions, and use 'GetElementPtr' and 'BitCast' instructions to enhance the ability of correlation extraction.
This correlation is the key to correct data dependency analysis.}
\lhm{The \emph{second} difficulty is how to distinguish between main-loop's input variables and local variables, since local variables defined in functions may share names with main-loop's input variables.
We address this problem based on an observation of local variables defined within functions are first allocated memory with 'Alloca' instructions on the stack, and we can capture local variables based on this feature.}
The \emph{third} difficulty is caused by conditional instructions when different conditional branches can be taken, and the analytical model must be able to capture and aggregate data dependencies in different branches. 
We propose a \emph{branch fusion engine} to integrate data dependencies from different conditional branches.
\end{comment}
% found in the main computation loop. If there are different branches in the main computation loop, we need to judge whether there are calculations in these branches and record the data dependencies between variables (output variables from preprocessing).}
% \az{TODO: removal: The other difficulty results from global variables, although global variables can cause critical security risks~\cite{kil2006address} and should be avoided in software engineering. 
% In particular, some main-loop’s inputs variables are found to be global variables.
% It is difficult to capture data dependency on global variables where the register name is a whitespace when the global variable is . 
% We design a value-matching mechanism to track data dependency on global variables.}

% The \emph{third} difficulty is to TODO: identify arithmetic variables that defined and participate in computations from a variety of application state, such as temporary registers, index notations, branch labels, and function names. 
% We address this problem based on an observation of a pattern that arithmetic variables always appear in memory operations, such as `Load' and `Store'. 
% We propose an \emph{operation pattern matching engine} that successfully identifies arithmetic variables. 
% In the trace, register names take many forms, such as number, character, whitespace, and String.
% It is difficult to find out the variables (called as arithmetic variables) that involved in computation through the register name.
% We propose a method to identify arithmetic variables based on instruction type matching}
% \lhm{In addition, the existence of global variables is different from that of local variables in the dynamic instruction execution trace. We need to provide a unique identification method for global variables.}

% \az{Move the different branches of computations to Step 2 in Section XXX.}
% 2) uninitialized global varialbes,
% 3) different branches of computations are taken across iterations of the main computation loop.

% There are a couple of difficulties in data dependency analysis. 
% First, there some variables are defined in the main loop, and they are used to store the results of the variables that defined before the main loop. During dependency analysis, we only consider 
% the variables defined outside the main loop, so we would lose some dependencies if they occurred with local variables. 
% In order to solve it, when we find a local variable is used to store the result of a computation, we will record the dependencies between this local variable and those variables involved in the computation, and then when the local variable is used again, we will replace it with those variables involved in the computation.
% \lhm{Second, if a function with parameters is called in the main loop, it is a challenge to determine which variables correspond to these parameters when the function is called. We have solved this problem using a stack (LIFO), which we will explain in detail in Section IV.}

% \az{how to handle for-loops in DDG analysis? }

\subsection{Identification of variables to checkpoint}
To identify variables to checkpoint from the \emph{contracted} DDG, which only includes the main computation loop's input variables, we summarize four data dependency types found at individual variables from data dependency analysis.
Those four dependency types are write-after-read, outcome, partially-overwritten, and fully-overwritten, from which we can determine whether to checkpoint a variable or not.
In particular, we do checkpoint to write-after-read, outcome, and partially-overwritten; we don't checkpoint fully-overwritten. 
In addition, we checkpoint the indexation of the main computation loop. 
% There is a challenges at this step.
% For some variables, which are uninitialized arrays, we cannot know the array size, such that we cannot determine if those arrays are fully or partially overwritten in some cases. 
% To be conservative, we checkpoint all those variables that are uninitialized arrays.
% , which we cannot determine the size.

\subsection{Manual development}
% \kt{Once we identify variables to checkpoint, how to incorporate the C/R scheme into a target program ?}
Our analysis tool outputs the variables to checkpoint, including the variable's name and locations (line numbers) in the source code. The output information  suggests programmers to easily add C/R code to those variables in the source code to quickly enable C/R.
%Unfortunately, we don't yet support automatically enabling C/R code to those variables right now,
%which will be our \textbf{future work}.
%We suggest programmers to manually add C/R code to those variables in the source code to enable C/R.
% (line number of source code).
% Programmers can modify applications to checkpoint applications using checkpoint libraries (such as FTI, Veloc, SCR, etc.) for fault tolerance of HPC applications based on the output information from our analysis model.


% \subsection{Limitations}
% Currently \texttt{AutoCheck} only works for C/C++ programs because 
% \texttt{AutoCheck} is built on LLVM/Clang techniques, which only support code generation for the C language family.
% As a result, we only evaluate \texttt{AutoCheck} on 13 benchmarks in C/C++ with OpenMP and MPI. 
% We keep it for future work to extend the AutoCheck approach to more programming languages, such as Python, and libraries, such as PyTorch.  

\begin{comment}
This is the first time we read the trace, we will store the part that needs to be analyzed for data dependencies from the trace file into memory.
Firstly, we need to distinguish the trace outside the main computation loop and inside the main computation loop, because for different parts of the trace, we have different ways to deal with.
As show in Figure~\ref{fig:example_code}, we divide the source code into three segments.
Secondly, if the trace belongs to outside of the main computation loop, we collect all the variables appear in the trace.
If the trace belongs to the inside of the main computation loop, not only do we need to collect the variables used within the main computation loop, we also need to store the traces generated within the main computation loop into memory for data dependency analysis, as it takes a lot of time to read the traces from the file.
Then, we need to match the variables that collected from the outside and inside of the main computation loop, in order to screen the variables that defined outside of the main computation loop and used both outside and inside of the main computation loop. 
Finally, the pre-processing module will output the variables that matched successfully and the trace within the main computation loop, which are used as the input of the data dependency analysis module.


%and the second time will start the data dependency analysis of the trace generated by main computation loop with the collected variables. Therefore, before performing data dependency analysis, we need to perform a pre-processing of the trace. Pre-processing is the first time we read the trace. In the preprocessing, we mainly do the following two things. (a) According to our study of trace, we found that all variables defined in the source code will have registers with the same name in trace. So we can use this feature of trace to collect the variables that are defined outside the main computation loop and used in the main computation loop from trace. (b) Since all instructions exist as strings in the trace file, it is not convenient for us to read the main computation loop trace for the second time for data dependency analysis. Therefore, we need to process the traces generated by the main computation loop into a more stable format for our analysis. 


2) Dependency Graph Construction: 
In computer science, dependency graph represents a graph in which several objects depend on each other.
% As shown in the Figure~\ref{fig:dependency_graph}, we construct a dependency graph by analyzing the data dependencies of the variables inside the main computation loop.
We construct a dependency graph between variables in the main computation loop through data dependency analysis.
During dependency analysis, we analysis the instructions one by one.
Firstly, we identify the operation type of the instruction according to the opcode.
Secondly, we identify which variables the instruction operates on.
Then, we correspond the operation type of the instruction with the variable it operates on to determine what we should do with this instruction(
\lhm{update the reg-var map, insert dependency to dependency graph or get dependency out of this instruction, we will describe these operations in detail in the Section IV.}).
Finally, we can collect all the dependencies between the variables that we obtain from pre-processing.
\lhm{After the data dependency analysis, \texttt{AutoCheck} generates a dependency graph as shown in the Figure~\ref{fig:dependency_graph} with the dependencies between the variables in the main computation loop. From the dependency graph, we can infer the variables for checkpointing in the main computation loop.}

%In computer science, dependency graph represents a graph in which several objects depend on each other. As shown in the Figure~\ref{dependency graph}, we construct a dependency graph by analyzing the data dependencies of the variables inside the main computation loop. After finishing the pre-processing, we start analyzing the traces generated by the main computation loop. In this part of the traces, we analyze the dependencies of the variables we collected in the pre-processing. Then, using the analyzed data dependencies to construct a dependency graph. From the dependency graph, we can infer the variables for checkpointing in the main computation loop.






3) Identification of Variables for Checkpointing: 
\lhm{We classify the variables in the main computation loop into five categories according to their read and write situations, which are write-after-read, partially-overwritten, fully-overwritten, output, and other case.
The variables classified to write-after-read, partially-overwritten, and output are the critical variables that identified as the output of \texttt{AutoCheck}, they all need to checkpoint.}
After the data dependency analysis, we start to analyze each dependency collected.
Firstly, we get the read and write status of variables from the dependencies.
Then, we classify the variables by their read and write status.
Finally, output the variables for checkpoint.
\end{comment}
%Usually, in an iterative program, most of the time is spent processing the main computation loop, so we only need to checkpoint those variables that are used in the main computation loop. when the program fails, restart the program with the last saved checkpoint files. when we finish the data dependency analysis, we can know all variables' situation of write and read that collected through pre-processing. Then, We classfy the variables into five categories through the situation of write and read. The five types we defined are write-after-read, partial-overwritten, fully-overwritten, out-put, others. Within these five types, variables classified as writer-after-read, partial-overwritten and output are used as the output of our tool, this part of variables are identified for checkpoting. In the section of design, we will describe these five types in detail.

% Currently our tool only supports the analysis of serial program‘s trace. As for the analysis of parallel program's trace, which is our future work.




==> rebuttal.tex <==
We thank the reviewers for their insightful comments and suggestions. Our answers are as follows.\\

\textbf{Reviewer \#1:}
\\
Q1:  The authors should try to explain better the discussion about partially-overwritten variables.\\

Thank you very much for your suggestion. We will add more details to it.\\
\\
Q2: Would it be possible to have more formal arguments to show that the proposed solution is correct?\\

Our solution is the first of its kind. We strive to find benchmarks for checkpointing variables but could not find one. We have tried our best to verify the correctness of our solution.\\

\textbf{Reviewer \#2:}
\\
Q1: Authors state in the introduction that AutoCheck is a complement to existing C/R libraries and extends them but do not explain how. Experiments show results for AutoCheck only. I wonder if it means that AutoCheck can provide the right variables to checkpoint. That way, it complements but does not extend libraries.\\

%Sorry for the confusion. AutoCheck is a complement to existing C/R libraries in the way that AutoCheck generates checkpointing variables and pass over to C/R libraries/developers. We keep it for future work to extend C/R libraries to integrate AutoCheck. We will amend the introduction and other related sections accordingly to reflect this clarification. \\

Sorry for the confusion.AutoCheck functions as an addition to current C/R libraries by producing checkpointing variables and transferring them to C/R libraries or developers. We keep it for future work to extend C/R libraries to integrate AutoCheck.We will adjust the introduction and other relevant sections to accurately convey this clarification.


\\
Q2: What happens when using programs that are not using a Bulk Synchronous Parallel model? For me, you cannot say that AutoCheck works with MPI if it only works when using 1 process. How do you handle MPI communication? For example, it is unclear how AutoCheck detects communications that should be re-issued. Please explain more.\\
%\zwp{first}

AutoCheck relies on the data dependency among the main loop input (MLI) variables to identify checkpointing variables, meaning it only seeks checkpointing variables from MLI variables. Even though new local variables may be introduced within the main loop by models like Bulk Synchronous Parallel (BSP) and non-BSP, along with complex communication patterns, the algorithmic meaning should remain consistent with the serial code to generate correct results. Consequently, the data dependency among the MLI variables is expected to remain intact regardless of any MPI parallelism such as BSP.

%AutoCheck is relying on the data dependency between the main loop input (MLI) variables to identify checkpointing variables (i.e., soliciting checkpointing variables only from MLI variables). 
%Although new (local) variables within the main loop could be introduced by Bulk Synchronous Parallel (BSP) model and non-BSP model and complicated communication patterns, the algorithmic semantics should retain the same as compared to the serial code to be able to generate correct results. 
%In consequence, the data dependency between the MLI variables is expected to be identical/preserved correctly, independent of any MPI parallelism such as BSP. 

\\
Q3: "Note that arguments and parameters to function calls cannot be temporary registers and must be variables": Why?\\

%Thank you very much for pointing it out. This argument is wrong. What we want to say is that we want to connect arguments and parameters (both are temporary registers) to their corresponding variables; we cannot capture the data dependency between variables from the temporary register mappings. We will amend the related section accordingly. \\

Thank you very much for pointing it out. This argument is wrong.What we're trying to express is the need to connect arguments and parameters (both of which are temporary registers) to their corresponding variables. However, it's not possible to determine the data dependency between variables solely from the mappings of temporary registers. We will amend the related section accordingly.
\\
Q4: In the results section, how did you identify the main loop in each benchmark? What happens if we give the wrong main loop to AutoCheck? Is it possible to have multiple main loops?\\

We manually find the main loop to be the most computationally demanding and longest-running loop. Autocheck works with any loop, but each loop will produce distinct checkpointing variables. It's possible to have multiple loops when pinpointing the main loop is is hard to identify. In such cases, AutoCheck can handle them one at a time. 
%We manually find the main loop to be the most computationally intensive and longest executing loop. Autocheck works with any loop, but different loops will generate different checkpointing variables. Yes, there can be multiple loops when the main loop is hard to identify. For multiple loops, AutoCheck can handle them one at a time. 

\textbf{Reviewer \#3:}
\\
Q1: If a program is traced in serial (true for OMP and MPI) , how can one be certain that the same code regions are active? For example, producer/consumer patterns are easily identified as being poorly managed.\\
%\zwp{second}

I think you are referring to the non-Bulk Synchronous Parallel (BSP) model, which has complicated and non-deterministic communication patterns. Please refer to Q2 for Reviewer #2.

%AutoCheck records the execution of programs and instruction-level operations in different environments and to analyse and identify them at the end of program execution, so serial tracing does not affect the use of Autocheck.\\
\\
Q2: What if what needs to be checkpointed is a complex data structure; can one pinpoint struct members specifically?\\
    
AutoCheck can identify the whole data structure but cannot pinpoint struct members specifically. We keep that for future work.\\

\textbf{Reviewer \#4:}
\\
Q1: Once the LLVM Flang Fortran front-end is ready, what is required to extend your tool to support Fortran using it?\\


AutoCheck relies on LLVM-tracer to generate a dynamic LLVM IR trace, utilizing LLVM IR as its input. There's a possibility of extending LLVM-Tracer to accommodate Fortran with Flang-generated LLVM IR. However, certain distinct Flang IR instructions need to be addressed first.
\\
Q2: How does your tool work with OpenMP tasks or target offload? Can you tool support Kokkos using the Pthread, CUDA, HIP or SYCL back-ends?\\

AutoCheck cannot work with these cases so far. We would like to support them in future work.\\

\textbf{Reviewer \#5:}
\\
Q1: Parallelization Overhead: While the paper discusses the benefits of OpenMP parallelization, it could further explore the overhead and potential limitations introduced by parallel processing in different environments e.g. MPI.\\

Thank you very much for your suggestion. We will explore that in future work.\\

